Two-Stage LASSO ADMM Signal Detection Algorithm For Large Scale MIMO

This paper explores the benefit of using some of the machine learning techniques and Big data optimization tools in approximating maximum likelihood (ML) detection of Large Scale MIMO systems. First, large scale MIMO detection problem is formulated as a LASSO (Least Absolute Shrinkage and Selection Operator) optimization problem. Then, Alternating Direction Method of Multipliers (ADMM) is considered in solving this problem. The choice of ADMM is motivated by its ability of solving convex optimization problems by breaking them into smaller sub-problems, each of which are then easier to handle. Further improvement is obtained using two stages of LASSO with interference cancellation from the first stage. The proposed algorithm is investigated at various modulation techniques with different number of antennas. It is also compared with widely used algorithms in this field. Simulation results demonstrate the efficacy of the proposed algorithm for both uncoded and coded cases.

==> sec01_intro.tex <==
\begin{abstract}
In this paper, we present a low complexity detection algorithm that is based on a LASSO (least absolute shrinkage and selection operator) estimation. It provides better trade-offs between complexity and performance, especially in large-scale MIMO systems. It also achieves better bit error rate (BER) performance than known heuristic algorithms in large-scale MIMO literature, such as Local Ascent Search and Reactive Tabu Search algorithms, especially at higher-order modulations. We further proposed two stage LASSO with the concept of interference cancellation and also with the concept of shadow area constraints as a measure of symbols reliability  to improve the detection accuracy. We evaluate both LASSO and 2-LASSO, and we compare them with state-of-art detection methods. Computer simulations demonstrate the efficacy of the proposed algorithm in large-scale MIMO systems for both uncoded and turbo coded cases.   
\end{abstract}

\section{Introduction}
\label{sec:intro}
The use of a large number of antennas at the transmitter and receiver becomes of interest in MIMO systems, due to the possibility of gaining high spectral efficiencies without the need for increasing bandwidth \cite{foschini1998limits}, \cite{bolcskei2004principles}, \cite{rusek2013scaling}. This interest poses challenges in several design aspects of MIMO systems, such as channel estimation, hardware implementation, and detection complexity \cite{rusek2013scaling}. In MIMO systems, the detector is often the bottleneck for the overall performance and complexity, and it is obviously exacerbated in the large-scale MIMO case. There have been many linear detectors and near-Maximum Likelihood (ML) detectors proposed in the literature of conventional ('small') MIMO systems; however, they become noncompetitive when used to serve large-scale systems because either they require prohibited complexity or their performance is deteriorated \cite{mohammed2009high}.\\
\indent Various algorithms have been presented in the literature that exhibit a large-system behavior where the BER performance improves and becomes increasingly closer to the ML performance as the number of antennas increases. A family of low complexity detectors called Likelihood Ascent Search (LAS) detectors have been proposed in \cite{vishnu2008low},\cite{li2010multiple},\cite{mohammed2009high} for large-scale MIMO systems. They are based on successively searching the local neighborhood of some good initial vectors, such as MMSE vector. They have also been generalized for higher order modulations and showed increased performance as the number of antennas increases; however, they still suffer from performance deterioration as the modulation order increases\cite{li2010multiple}. Another neighborhood search algorithm that is based on reactive tabu search (RTS) \cite{battiti1994reactive} has also been proposed for large-scale MIMO systems with various QAMs in \cite{rajan2009low},\cite{srinidhi2009near},\cite{datta2010random}. This algorithm is a heuristic based combinatorial optimization technique which achieves near-ML performance with much lower complexity compared to ML and sphere decoder. However, its computational complexity scales up significantly with increasing QAM modulation levels accompanied with performance deterioration. There have been a few other detection algorithms that were presented for large-scale MIMO systems and shown to achieve near-optimal performance, but only for $ \left\lbrace -1, 1\right\rbrace  $ alphabet, such as the work in \cite{hansen2009near}, and in \cite{som2010improved}.\\

\indent In this paper, we re-formulate ML problem into LASSO (least absolute shrinkage and selection operator) optimization problem. LASSO (\cite{tibshirani1996regression}), is a regression analysis method that has been widely used in machine learning and big data optimization. It performs both variable selection and regularization in order to enhance the prediction accuracy and interpretability of the statistical model. Motivated by the success of LASSO in performing high dimensional data clustering (\cite{elhamifar2013sparse}), and by the similarity of Large scale MIMO detection problem to high dimensional dataset classification, and we investigate the use of LASSO in large scale MIMO detection.

\indent Our choice of LASSO is motivated by the fact that every received symbol can be represented as a sparse linear combination of the modulated symbols. However, ideally there will be only one non zero coefficient with a value that is exactly equal to one and all other coefficients are zeros. In the presence of noise and channel effect, There could be many non zero coefficients, but the symbol with the highest coefficient is the best approximate to the ML estimate of the received symbol.

\indent To further improve the accuracy of the LASSO estimation, we implement 2 stage LASSO (2-LASSO). The idea of this algorithm is to implement two stages of LASSO detection with interference cancellation to further improve the detection of the unreliable symbols. In the first round, symbols with only one large coefficient are quantized to the nearest symbol and LASSO is implemented for the second time after removing the contribution of the detected symbols. This novel idea helps removing the interference from other symbols and increasing the detection accuracy with the cost of little bit higher complexity.

\indent LASSO is a convex optimization problem which can be solved using any generic convex solver. However, we choose to solve it using ADMM (alternating direction method of multipliers) because ADMM takes the advantage of the separability of the LASSO objective function and the different structure of the two summed functions (quadratic and norm 1) and break the problem into pieces, each of which are solved differently. It is a widely used algorithm for solving separable convex optimization problems with linear constraints. Global convergence of ADMM was established in the early 1990’s by Eckstein and Bertsekas \cite{Eckstein:1992:DSM:153390.153393}.  The interest in ADMM has exploded in recent years because of applications in signal and image processing, compressed sensing \cite{2009arXiv0912.1185Y}, matrix completion \cite{Yuan:2009vu}, distributed optimization, and statistical machine learning \cite{Boyd:2011:DOS:2185815.2185816}, and quadratic and linear programming \cite{doi:10.1137/120878951}.

\if 0
\indent Conventional quadratic programming detectors, which is based on reformulating the ML problem into a quadratic optimization problem, are already studied in conventional MIMO systems \cite{bhatti2011mimo}, \cite{zhang2007integer}, \cite{mobasher2007near}, \cite{elghariani2012QAM}, and other large-scale systems, such as Spread OFDM \cite{c9}. However, we note a lack of performance comparisons in the literature of large-scale MIMO systems with the existing heuristic search techniques. In this paper, we study via simulation the performance and complexity of the conventional QP detector in large-scale MIMO systems and point out that it is one of the detectors that exhibit large-system behavior. Thus any other algorithm that is based on QP can have the same behavior in the large-scale systems. \\
\indent The proposed algorithm in this paper improves the performance of the conventional QP detectors with a minor complexity increase. It is based on the use of a two-stage quadratic programming detector with a novel combination of a successive interference cancellation strategy and a symbol reliability measure that utilizes a shadow area constraint \cite{lamar2011multiple}. \\
\indent A motivation to why we suggest the QP based detectors in the large-scale MIMO is as follows. Both LAS and RTS family of algorithms are based on searching a local neighborhood of some starting initial vector, such as MMSE. The LAS algorithm sticks with the first local minima it finds, while RTS algorithm escapes to several other local minimas and then selects the minimum one among all. On the other hand, QP solvers, such as the interior-point algorithm \cite{rao1998application}, which we will use in this paper, finds a global minima, but in the continuous sense (non-integer solution). Therefore, we show in this work that in large-scale MIMO detection problems, solving a QP optimization problem could be more efficient than performing a heuristic search.  
\fi



